Load Balancing-based Topology Adaptation for Integrated Access and Backhaul Networks

Integrated access and backhaul (IAB) technology is a flexible solution for network densification. IAB nodes can also be deployed in moving nodes such as buses and trains, i.e., mobile IAB (mIAB). As mIAB nodes can move around the coverage area, the connection between mIAB nodes and their parent macro base stations (BSs), IAB donor, is sometimes required to change in order to keep an acceptable backhaul link, the so called topology adaptation (TA). The change from one IAB donor to another may strongly impact the system load distribution, possibly causing unsatisfactory backhaul service due to the lack of radio resources. Based on this, TA should consider both backhaul link quality and traffic load. In this work, we propose a load balancing algorithm based on TA for IAB networks, and compare it with an approach in which TA is triggered based on reference signal received power (RSRP) only. The results show that our proposed algorithm improves the passengers worst connections throughput in uplink (UL) and, more modestly, also in downlink (DL), without impairing the pedestrian quality of service (QoS) significantly.

==> acronyms.tex <==
\acro{2D}{Two-Dimensional}
\acro{3D}{Three-Dimensional}
\acro{4D}{Four-Dimensional}
\acro{6D}{Six-Dimensional}
\acro{1G}{First Generation}
\acro{2G}{Second Generation}
\acro{3G}{Third Generation}
\acro{4G}{Fourth Generation}
\acro{5G}{Fifth Generation}
\acro{5GC}{5G Core Network}
\acro{5G-StoRM}{5G Stochastic Radio Channel for Dual Mobility}
\acro{6G}{Sixth Generation}
\acro{3GPP}{3rd Generation Partnership Project}
\acro{3GPP2}{3rd Generation Partnership Project 2}
\acro{A2A}{Air-to-Air}
\acro{A2G}{Air-to-Ground}
\acro{AA}{Antenna Array}
\acro{AC}{Admission Control}
\acro{AD}{Attack-Decay}
\acro{AE}{Antenna Element}
\acro{AF}{Amplify and Forward}
\acro{ABS}{Almost Blank Subframe}
\acro{ACF}{Autocorrelation Function}
\acro{ADSL}{Asymmetric Digital Subscriber Line}
\acro{AHW}{Alternate Hop-and-Wait}
\acro{AI}{Artificial Intelligence}
\acro{AMC}{Adaptive Modulation and Coding}
\acro{AP}{Access Point}
\acro{APA}{Adaptive Power Allocation}
\acro{API}{Application Protocol Interface}
\acro{ARQ}{Automatic Repeat Request}
\acro{AT}{averaged time}
\acro{ARMA}{Autoregressive Moving Average}
\acro{ASE}{Average Squared Error}
\acro{ASC}{Adaptive Satisfaction Control}
\acro{ATES}{Adaptive Throughput-based Efficiency-Satisfaction Trade-Off}
\acro{AWGN}{Additive White Gaussian Noise}
\acro{BAP}{Backhaul Adaptation Protocol}
\acro{BB}{Branch and Bound}
\acro{BC}{Branch and Cut}
\acro{BD}{Block Diagonalization}
\acro{BER}{Bit Error Rate}
\acro{BF}{Best Fit}
\acro{BL}{Bit Loading}
\acro{BLER}{BLock Error Rate}
\acro{BLPC-1}{Bit Loading with Power Constraint in Hop 1}
\acro{BLPC-2}{Bit Loading with Power Constraint in Hop 2}
\acro{BPC}{Binary Power Control}
\acro{BPSK}{Binary Phase-Shift Keying}
\acro{BRA}{Balanced Random Allocation}
\acro{BS}{Base Station}
\acro{BSP}{\acs*{BS} Placement}
\acro{BSR}{Buffer Status Report}
\acro{CAP}{Combinatorial Allocation Problem}
\acro{CAPEX}{Capital Expenditure}
\acro{CB}{Contextual Bandit}
\acro{CBF}{Coordinated Beamforming}
\acro{CBR}{Constant Bit Rate}
\acro{CBS}{Class Based Scheduling}
\acro{CC}{Congestion Control}
\acro{CCL}{Common Cell List}
\acro{CDF}{Cumulative Distribution Function}
\acro{CDL}{Clustered Delay Line}
\acro{CDMA}{Code-Division Multiple Access}
\acro{CIR}{channel impulse response}
\acro{CH}{Channel Hardening}
\acro{CHO}{Conditional Handover}
\acro{C-RAN}{cloud-based Radio Access Network}
\acro{CL}{Closed Loop}
\acro{CLT}{central limit theorem}
\acro{CLPC}{Closed Loop Power Control} 
\acro{CN}{Core Network}       
\acro{CNR}{Channel-to-Noise Ratio}
\acro{CP}{Control Plane}
\acro{CPA}{Cellular Protection Algorithm}
\acro{CPICH}{Common Pilot Channel}
\acro{CoMP}{Coordinated Multi-Point}
\acro{CQI}{Channel Quality Indicator}
\acro{CRE}{Cell Range Expansion}
\acro{CRM}{Constrained Rate Maximization}
\acro{CRN}{Cognitive Radio Network}
\acro{C-RNTI}{Cell Radio Network Temporary Identifier}
\acro{CRRM}{Centralized/Common Radio Resource Management}
\acro{CRS}{Cell-specific Reference Signal}
\acro{CS}{Coordinated Scheduling}
\acro{CSI}{Channel State Information}
\acro{CSI-RS}{Channel State Information Reference Signal}
\acro{CTS}{Clear to Send}
\acro{CU}{Centralized Unit}
\acro{CUE}{Cellular User Equipment}
\acro{CWND}{Congestion window size}
\acro{D2D}{Device-to-Device}
\acro{D2N}{Drone-to-Network}
\acro{DAA}{Drone Antenna Array}
\acro{DAG}{Directed Acyclic Graph}
\acro{DBS}{Drone Mounted Base Station}
\acro{DC}{Dual Connectivity}
\acro{DCA}{Dynamic Channel Allocation}
\acro{DE}{Differential Evolution}
\acro{DF}{Decode and Forward}
\acro{DFT}{Discrete Fourier Transform}
%\acro{DIST}{Distance-based Grouping}
\acro{DIST}{Distance}
\acro{DL}{Downlink}
\acro{DMA}{Double Moving Average}
\acro{DMRS}{Demodulation Reference Signal}
\acro{D2DM}{\acs*{D2D} Mode}
\acro{DMS}{\acs*{D2D} Mode Selection}
\acro{DP}{Data Plane}
\acro{DPC}{Dirty Paper Coding}
\acro{DRA}{Dynamic Resource Assignment}
\acro{DSA}{Dynamic Spectrum Access}
\acro{DSM}{Delay-based Satisfaction Maximization}
\acro{DU}{Distributed Unit}
\acro{E2E}{End-to-End}
\acro{ECC}{Electronic Communications Committee}
\acro{EDF}{Earliest Deadline First}
\acro{EE}{Energy Efficiency}
\acro{EFLC}{Error Feedback Based Load Control}
\acro{EI}{Efficiency Indicator}
\acro{e-ICIC}{Enhanced Inter-Cell Interference Coordination}
\acro{eMBB}{Enhanced Mobile Broadband}
\acro{eNB}{Evolved Node B}
\acro{EXP}{Exponential}
\acro{EPA}{Equal Power Allocation}
\acro{EPC}{Evolved Packet Core}
\acro{EPS}{Evolved Packet System}
\acro{E-UTRAN}{Evolved Universal Terrestrial Radio Access Network}
\acro{ES}{Exhaustive Search}
\acro{FCP}{Fundamental Counting Principle}
\acro{FCA}{Flow Control Algorithm}
\acro{FD}{Full Duplex}
\acro{FDD}{Frequency Division Duplex}
\acro{FDM}{Frequency Division Multiplexing}
\acro{FDMA}{Frequency Division Multiple Access}
\acro{FER}{Frame Erasure Rate}
\acro{FoV}{Field-of-view}
\acro{FIFO}{First In First Out}
\acro{FF}{Fast Fading}
\acro{FR}{Frequency Range}
\acro{FRS}[FS]{Fast-RAT Scheduling}
\acro{FS}{Fast Switching}
\acro{FSB}{Fixed Switched Beamforming}
\acro{FST}{Fixed \acs*{SNR} Target}
\acro{FT}{Fourier transform}
\acro{FTP}{File Transfer Protocol}
\acro{Fwd}{Forwarding}
\acro{GA}{Genetic Algorithm}
\acro{GAP}{Generalized Assignment Problem}
\acro{GAP-MQ}{Generalized Assignment Problem with Minimum Quantities}
\acro{GATES}{Generalized Adaptive Throughput-based Efficiency-Satisfaction Trade-Off}
\acro{GBR}{Guaranteed Bit Rate}
\acro{GLR}{Gain to Leakage Ratio}
\acro{gNB}{gNodeB}
\acro{GOS}{Generated Orthogonal Sequence}
\acro{GP}{Gaussian Process}
\acro{GPL}{GNU General Public License}
\acro{GPS}{Global Positioning System}
\acro{GRP}{Grouping}
\acro{GSM}{Global System for Mobile Communications}
\acro{GTEL}{Wireless Telecommunications Research Group}
\acro{HARQ}{Hybrid Automatic Repeat Request}
\acro{HBF}{Hybrid Beamforming}
\acro{HCPP}{Hardcore Point Process}
%\acro{HD}{High Definition}
\acro{HetNet}{Heterogeneous Network}
\acro{HD}{Half Duplex}
\acro{HH}{Hughes-Hartogs}
\acro{HardH}[HH]{Hard Handover}
\acro{HMS}{Harmonic Mode Selection}
\acro{HO}{Handover}
\acro{HOL}{Head Of Line}
\acro{HPBW}{Half Power Beamwidth}
\acro{HSDPA}{High Speed Downlink Packet Access}
\acro{HSR}{High-Speed Railway}
\acro{HSPA}{High Speed Packet Access}
\acro{HTTP}{HyperText Transfer Protocol}
\acro{IAB}{Integrated Access and Backhaul}
\acro{ICMP}{Internet Control Message Protocol} 
\acro{ICI}{Intercell Interference}
\acro{ICIC}{Inter-Cell Interference Coordination}
\acro{ID}{Identification}
\acro{i.i.d.}{independent and identically distributed}
\acro{IETF}{Internet Engineering Task Force}
\acro{IPC}{Individual Power Constraint}
%\acro{ILP}{Integer Linear Program}
\acro{UID}{Unique Identification}
\acro{IID}{Independent and Identically Distributed}
\acro{IIR}{Infinite Impulse Response}
\acro{ILP}{Integer Linear Problem}
\acro{IMT}{International Mobile Telecommunications}
\acro{INV}{Inverted Norm-based Grouping} 
\acro{IoT}{Internet of Things}
\acro{IP}{Internet Protocol}
\acro{IPv6}{Internet Protocol Version 6}
\acro{IRA}{Integrated Resource Allocation}
\acro{IRS}{Intelligent Reflecting Surface}
\acro{ISAC}{Integrated Sensing And Communication}
\acro{ISD}{Inter-Site Distance}
\acro{ISI}{Inter Symbol Interference}
\acro{ISM}{Industrial, Scientific and Medical}
\acro{ITU}{International Telecommunication Union}
\acro{JOAS}{Joint Opportunistic Assignment and Scheduling}
\acro{JOS}{Joint Opportunistic Scheduling}
\acro{JP}{Joint Processing}
\acro{JRAPAP}{Joint RB Assignment and Power Allocation Problem}
\acro{JS}{Jump-Stay}
\acro{JSM}{Joint Satisfaction Maximization}
\acro{KKT}{Karush-Kuhn-Tucker}
\acro{KPI}{Key Performance Indicator}
\acro{LAC}{Link Admission Control}
\acro{LA}{Link Adaptation}
\acro{LBS}{Location Based Service}
\acro{LC}{Load Control}
\acro{LOS}{Line of Sight}
\acro{LP}{Linear Programming}
\acro{LTE}{Long Term Evolution}
\acro{LTE-A}{\acs*{LTE}-Advanced}
\acro{LTE-Advanced}{\ac{LTE-A}}
\acro{LTE-R}{\ac{LTE} Railway}
\acro{LSP}{Large Scale Parameter}
\acro{MADRDPG}{Multi-Agent Deep Recurrent Deterministic Policy Gradient}
\acro{MeNB}{Master \acs*{eNB}}
\acro{M2M}{Machine-to-Machine}
\acro{MAC}{Medium Access Control}
\acro{MANET}{Mobile Ad hoc Network}
\acro{MEDS}{Method of Exact Doppler Spread}
\acro{MC}{Modular Clock}
\acro{MCP}{Minimal Cost Power}
\acro{MCS}{Modulation and Coding Scheme}
\acro{MDB}{Measured Delay Based}
\acro{MDI}{Minimum \acs*{D2D} Interference}
\acro{MDSM}{Modified Delay-based Satisfaction Maximization}
\acro{MDU}{Max-Delay-Utility}
\acro{METIS}{Mobile and Wireless Communications Enablers for the Twenty-twenty Information Society \acs*{5G}}
\acro{MF}{Matched Filter}
\acro{MFAP}{Mobile Femtocell Access Point}
\acro{MG}{Maximum Gain}
\acro{MH}{Multi-Hop}
\acro{mIAB}{Mobile \ac{IAB}}
\acro{MILP}{Mixed Integer Linear Programming}
\acro{MIMO}{Multiple Input Multiple Output}
\acro{MINLP}{Mixed Integer Nonlinear Programming}
\acro{MIP}{Mixed Integer Programming}
\acro{MISO}{Multiple Input Single Output}
\acro{MIT}{Mobility Interruption Time}
\acro{ML}{Machine Learning}
\acro{MLWDF}{Modified Largest Weighted Delay First}
\acro{MME}{Mobility Management Entity}
\acro{MMF}{Max-Min Fairness}
\acro{mmMAGIC}{Millimetre-Wave Based Mobile Radio Access Network for Fifth Generation Integrated Communications}
\acro{MMRP}{Maximizing the Minimal Residual Power}
\acro{MMRP-LB}{Maximizing the Minimal Residual Power with Lower Bound}
\acro{MMSE}{Minimum Mean Square Error}
\acro{mMTC}{Massive Machine-Type Communications}
\acro{mmWave}{millimeter Wave}
\acro{MN}{Master Node}
\acro{MOS}{Mean Opinion Score}
\acro{MPF}{Multicarrier Proportional Fair}
\acro{MPRP}{Maximization of the Product of the Residual Powers}
\acro{MRA}{Maximum Rate Allocation}
\acro{MR}{Maximum Rate}
\acro{MRC}{Maximum Ratio Combining}
\acro{MRN}{Mobile Relay Node}
\acro{MRT}{Maximum Ratio Transmission}
\acro{MRUS}{Maximum Rate with User Satisfaction}
\acro{MS}{Mode Selection}
\acro{MSE}{Mean Squared Error}
\acro{MCG}{Master Cell Group} 
\acro{MSI}{Multi-Stream Interference}
\acro{MT}{Mobile Termination}
\acro{MTC}{Machine-Type Communication}
\acro{IMS}{\acs*{IP} Multimedia Subsystem}
\acro{MTSI}{Multimedia Telephony Services over \acs*{IMS}}
\acro{MTSM}{Modified Throughput-based Satisfaction Maximization}
\acro{MU-MIMO}{Multi-User Multiple Input Multiple Output}
\acro{MU}{Multi-User}
\acro{Multi-CUT}{Multi-Cell and Multi-User and Multi-Tier}
\acro{NAS}{Non-Access Stratum}
\acro{NB}{Node B}
\acro{nBS}{Neighbor Base Station}
\acro{NCL}{Neighbor Cell List}
\acro{NCR}{Network-Controlled Repeater}
\acro{NG}{Next Generation Core}
\acro{NGC}{Next Generation Core Network}
\acro{NLP}{Nonlinear Programming}
\acro{NLOS}{Non-Line of Sight}
\acro{NMSE}{Normalized Mean Square Error}
\acro{NN}{Neural Network}
\acro{NOMA}{Non-Orthogonal Multiple Access}
\acro{NORM}{Normalized Projection-based Grouping}
\acro{NP}{Non-Polynomial Time}
\acro{NR}{New Radio}
\acro{NRT}{Non-Real Time}
\acro{NSA}{Non-Stand-Alone}
\acro{NSPS}{National Security and Public Safety Services}
%\acro{O2I}{Outdoor to Indoor}
\acro{OBF}{Opportunistic Beamforming}
\acro{OFDMA}{Orthogonal Frequency Division Multiple Access}
\acro{OFDM}{Orthogonal Frequency Division Multiplexing}
\acro{OFPC}{Open Loop with Fractional Path Loss Compensation}
\acro{O2I}{Outdoor-to-Indoor}
\acro{OL}{Open Loop}
\acro{OLPC}{Open-Loop Power Control}
\acro{OL-PC}{Open-Loop Power Control}
\acro{OM}[O\&M]{Operational \& Maintenance}
\acro{OMA}{Orthogonal Multiple Access}
\acro{OPEX}{Operational Expenditure}
\acro{ORA}{Orthogonal Resource Allocation}
\acro{ORB}{Orthogonal Random Beamforming}
\acro{OSM}{Open Street Map}
\acro{JO-PF}{Joint Opportunistic Proportional Fair}
\acro{OSI}{Open Systems Interconnection}
\acro{PA}{Power Allocation}
\acro{PAIR}{\acs*{D2D} Pair Gain-based Grouping}
\acro{PAPR}{Peak-to-Average Power Ratio}
\acro{P2P}{Peer-to-Peer}
\acro{PBCH}{Physical Broadcast Channel}
\acro{PBS}{Pico Base Station}        
\acro{PC}{Power Control}
\acro{PCI}{Physical Cell \acs*{ID}}
\acro{PDCP}{Packet Data Convergence Protocol}
\acro{PDF}{Probability Density Function}
\acro{PDU}{Protocol Data Unit}
\acro{PER}{Packet Error Rate}
\acro{PF}{Proportional Fair}
\acro{PGRA}{Probabilistic Graph based Resource Allocation}
\acro{P-GW}{Packet Data Network Gateway}
\acro{PHY}{Physical}
\acro{PL}{Pathloss}
\acro{PLR}{Packet Loss Ratio}
\acro{PRABE}{Power and Resource Allocation Based on Quality of Experience}
\acro{PRB}{Physical Resource Block}
\acro{PROJ}{Projection-based Grouping}
\acro{PSD}{Power Spectral Density}
\acro{PSDe}{positive semi-definite}
\acro{ProSe}{Proximity Services}
\acro{PS}{Packet Scheduling}
\acro{PSO}{Particle Swarm Optimization}
\acro{PSS}{Primary Synchronization Signal}
\acro{PTAS}{Polynomial-Time Approximation Scheme}
\acro{PTP}{Point-to-Point}
\acro{PZF}{Projected Zero-Forcing}
\acro{QAM}{Quadrature Amplitude Modulation}
\acro{QHMLWDF}{Queue-HOL-MLWDF}
\acro{QoE}{Quality of Experience}
\acro{QoS}{Quality of Service}
\acro{QPSK}{Quadri-Phase Shift Keying}
\acro{QSM}{Queue-based Satisfaction Maximization}
\acro{QuaDRiGa}{QUAsi Deterministic RadIo channel GenerAtor}
\acro{RACH}{Random Access}
\acro{RAISES}{Reallocation-based Assignment for Improved Spectral Efficiency and Satisfaction}
\acro{RAN}{Radio Access Network}
\acro{RA}{Resource Allocation}
\acro{RAP}{RB Assignment Problem}
\acro{RAT}{Radio Access Technology}[long-plural-form={Radio Access Technologies}]
\acro{RATE}{Rate-based}
\acro{RAU}{Remote Antenna Unit}
\acro{RB}{Resource Block}
\acro{RBG}{Resource Block Group}
\acro{REF}{Reference Grouping}
\acro{RET}{Remote Electrical Tilt}
\acro{RF}{Radio Frequency}
\acro{RL}{Reinforcement Learning}
\acro{RLC}{Radio Link Control}
\acro{RLF}{Radio Link Failure}
\acro{RM}{Rate Maximization}
\acro{RMa}{Rural Macro}
\acro{RMJ-SNR}{Region of the Minimum Joint SNR}
\acro{RMEC}{Rate Maximization under Experience Constraints}
\acro{RMSE}{root-mean-square error}
\acro{RNC}{Radio Network Controller}
\acro{RND}{Random Grouping}
\acro{RNN}{Recurrent Neural Network}
\acro{RRA}{Radio Resource Allocation}
\acro{RRM}{Radio Resource Management}
\acro{RSCP}{Received Signal Code Power}
\acro{RSRP}{Reference Signal Received Power}
\acro{RSRQ}{Reference Signal Received Quality}
\acro{RR}{Round Robin}
\acro{RRC}{Radio Resource Control}
\acro{RSSI}{Received Signal Strength Indicator}
\acro{RT}{Real Time}
\acro{RTR}[RT]{Ray-Tracing}
\acro{RTS}{Request to Send}
\acro{RU}{Resource Unit}
\acro{RUNE}{RUdimentary Network Emulator}
\acro{RV}{Random Variable}
\acro{Rx}{Receiver}
\acro{RZF}{Regularized Zero-Forcing}
\acro{SA}{Subcarrier Assignment}
\acro{SAC}{Session Admission Control}
\acro{sBS}{Serving Base Station}
\acro{SC}{Small Cell}
\acro{SCon}[SC]{Single Connectivity}
\acro{SCG}{Secondary Cell Group}
\acro{SCM}{Spatial Channel Model}
\acro{SCS}{Subcarrier Spacing}
\acro{SC-FDMA}{Single Carrier - Frequency Division Multiple Access}
\acro{SCRV}{Spatially Consistent Random Variable}
\acro{SD}{Soft Dropping}
\acro{SDAP}{Service	Data Adaptation Protocol}
\acro{S-D}{Source-Destination}
\acro{SDPC}{Soft Dropping Power Control}
\acro{SDM}{Space-Division Multiplexing}
\acro{SDMA}{Space-Division Multiple Access}
\acro{SE}{Squared Error}
\acro{SF}{Shadow Fading}
\acro{SMDP}{Semi-Markov	Decision Problem}
\acro{SeNB}{Secondary \acs*{eNB}}
\acro{SER}{Symbol Error Rate}
\acro{SES}{Simple Exponential Smoothing}
\acro{S-GW}{Serving Gateway}
\acro{SINR}{Signal to Interference-plus-Noise Ratio}
\acro{SLNR}{Signal to Leakage-plus-Noise Ratio}
\acro{SNN}{strictly non-negative}
\acro{SI}{Satisfaction Indicator}
\acro{SIC}{Successive Interference Cancellation}
\acro{SIP}{Session Initiation Protocol}
\acro{SISO}{Single Input Single Output}
\acro{SIMO}{Single Input Multiple Output}
\acro{SIR}{Signal to Interference Ratio}
\acro{SM}{Subcarrier Matching}
\acro{SMA}{Simple Moving Average}
\acro{SMSE}{spatial-mean-square error}
\acro{SN}{Secondary Node}
\acro{SNR}{Signal to Noise Ratio}
\acro{SON}{Self Organizing Networks}
\acro{SoA}{state-of-the-art}
\acro{SoS}{Sum-of-Sinusoids}
\acro{SORA}{Satisfaction Oriented Resource Allocation}
\acro{SORA-NRT}{Satisfaction-Oriented Resource Allocation for Non-Real Time Services}
\acro{SORA-RT}{Satisfaction-Oriented Resource Allocation for Real Time Services}
\acro{SP}{Signal Processing}
\acro{SPF}{Single-Carrier Proportional Fair}
\acro{SR}{Smart Repeater}
\acro{SRA}{Sequential Removal Algorithm}
\acro{SRB1}{Signaling Radio Bearer~1}
\acro{SRS}{Sounding Reference Signal}
\acro{SSB}{Synchronization Signal Block}
\acro{SSP}{Small Scale Parameter}
\acro{SSS}{Secondary Synchronization Signal}
\acro{ST}{Spanning Tree}
\acro{STTD}{Space Time Transmit Diversity}[long-plural-form={Space Time Transmit Diversities}]
\acro{SU-MIMO}{Single-User Multiple Input Multiple Output}
\acro{SU}{Single-User}
\acro{tBS}{Target Base Station}
\acro{SVD}{Singular Value Decomposition}
\acro{TCP}{Transmission Control Protocol}
\acro{TDD}{Time Division Duplex}
\acro{TDM}{Time Division Multiplexing}
\acro{TDMA}{Time Division Multiple Access}
\acro{TETRA}{Terrestrial Trunked Radio}
\acro{TP}{Transmit Power}
\acro{TPC}{Total Power Constraint}
%\acro{TPC}{Transmit Power Control}
\acro{TR}{Technical Report}
\acro{TTI}{Transmission Time Interval}
\acro{TTR}{Time-To-Rendezvous}
\acro{TTT}{Time-To-Trigger}
\acro{TSM}{Throughput-based Satisfaction Maximization}
\acro{TU}{Typical Urban}
\acro{TV}{Television}
\acro{TVWS}{\acs*{TV} White Space}
\acro{Tx}{Transmitter}
\acro{UAV}{Unmanned Aerial Vehicle}
\acro{UABSC}{User-Assisted Bearer Split Control}
\acro{UDP}{User Datagram Protocol}
\acro{UDN}{Ultra-Dense Networks}
\acro{UE}{User Equipment}
\acro{UBA}{\ac{UE}-\ac{BS} association}
\acro{UEPS}{Urgency and Efficiency-based Packet Scheduling}
\acro{UFC}{Federal University of Cear\'{a}}
\acro{ULA}{Uniform Linear Array}
\acro{UL}{Uplink}
\acro{UMa}{Urban Macro}
\acro{UMi}{Urban Micro}
\acro{UMTS}{Universal Mobile Telecommunications System}
\acro{UP}{User Plane}
\acro{UPN}{User Provided Network}
\acro{URA}{Uniform Rectangular Array}
\acro{URI}{Uniform Resource Identifier}
\acro{URLLC}{Ultra-Reliable Low-Latency Communications}
\acro{URM}{Unconstrained Rate Maximization}
\acro{VBR}{Variable Bit Rate}
\acro{VET}{Variable Electrical Tilt}
\acro{VMR}{Vehicle-Mounted Relay}
\acro{VR}{Virtual Resource}
\acro{VoIP}{Voice over \acs*{IP}}
\acro{WCDMA}{Wideband Code Division Multiple Access}
\acro{WF}{Water-filling}
\acro{WID}{Wireless Infrastructure Drone}
\acro{Wi-Fi}{Wireless Fidelity}
\acro{WiMAX}{Worldwide Interoperability for Microwave Access}
\acro{WINNER}{Wireless World Initiative New Radio}
\acro{WLAN}{Wireless Local Area Network}
\acro{WMPF}{Weighted Multicarrier Proportional Fair}
\acro{WP}{Work Package}
\acro{WPF}{Weighted Proportional Fair}
\acro{WSN}{Wireless Sensor Network}
\acro{WWW}{World Wide Web}
\acro{WFQ}{Weighted Fair Queuing}
\acro{XIXO}{(Single or Multiple) Input (Single or Multiple) Output}
\acro{XPR}{Cross-Polarization Power Ratio}
\acro{ZF}{Zero-Forcing}
\acro{ZMCSCG}{Zero Mean Circularly Symmetric Complex Gaussian}

